Construction of Knowledge Graphs: State and Challenges

With knowledge graphs (KGs) at the center of numerous applications such as recommender systems and question answering, the need for generalized pipelines to construct and continuously update such KGs is increasing. While the individual steps that are necessary to create KGs from unstructured (e.g. text) and structured data sources (e.g. databases) are mostly well-researched for their one-shot execution, their adoption for incremental KG updates and the interplay of the individual steps have hardly been investigated in a systematic manner so far. In this work, we first discuss the main graph models for KGs and introduce the major requirement for future KG construction pipelines. Next, we provide an overview of the necessary steps to build high-quality KGs, including cross-cutting topics such as metadata management, ontology development, and quality assurance. We then evaluate the state of the art of KG construction w.r.t the introduced requirements for specific popular KGs as well as some recent tools and strategies for KG construction. Finally, we identify areas in need of further research and improvement.

==> kg-tasks/evaluation.tex <==
The quality of a KG is crucial for its credibility and therefore its usability in applications~\cite{10.1080/07421222.1996.11518099}. 
Quality assurance is the task to maintain a high KG quality despite the continuous evolution of the KG. %to meet new requirements and remain up-to-date. 
It comprises quality evaluation as well as quality improvement \textbf{including knowledge completion} (Section \ref{sec:completion}). Quality evaluation serves to assess the quality and detect quality issues. Quality improvement aims at fixing or mitigating the detected quality issues by refining and repairing the KG. This encompasses inferring and adding missing knowledge to
the graph, or identifying and repairing erroneous pieces of information in order to improve data quality. 
Quality evaluation is not only important for the resulting KG as outcome of the KG construction process but also within the different construction tasks, such as data cleaning for acquired data, knowledge extraction, ontology evolution or entity fusion. 
The data cleaning approaches mentioned in Section \ref{sec:datacleaning} can also be applied to the KG, e.g. to identify outliers or contradicting information. 
Metadata such as provenance information is also important for quality assurance, for example to explain and maintain KG data concerning the context and validity of conflicting values~\cite{Weikum2021MachineKC}.

Different methods for \textbf{quality evaluation} have been proposed that can be categorized into internal and external methods~\cite{paulheim2017knowledge}.
\textit{Internal methods} only use the current KG for evaluation.
One conventional approach is to evaluate the accuracy of the KG against a manually labeled subset of entities and relations~\cite{paulheim2017knowledge}. However, this is costly, so that those gold standards are usually small. Other approaches use statistical methods such as distance-based, deviations-based and distribution based methods~\cite{bizer2009quality}. 

By contrast, \textit{external methods} also use external knowledge sources for quality evaluation such as crowdsourcing methods or other KGs.  

\begin{itemize}
\item \textbf{Crowdsourcing approaches}: 
Acosta et al.~\cite{acosta2013crowdsourcing} leverages the wisdom of the crowds in two ways. They launched a contest targeting an expert crowd in order to find and classify erroneous RDF triples, and then published the outcome of this contest as paid microtasks on Amazon Mechanical
Turk (MTurk) in order to verify the issues spotted by the experts. Their empirical evaluation on DBpedia shows that the two styles of crowdsourcing are complementary, and that crowdsourcing-enabled quality assessment is a promising and affordable way to enhance data quality. 

Paulheim et al.~\cite{paulheim2017knowledge} define \textit{retrospective evaluation} as a method in which the human judges the correctness of the KG The reported quality metric is accuracy or precision. Since KGs are often voluminous, the retrospective approach is typically restricted to a KG sample. 

\item \textbf{Using external knowledge bases}:
Li et al.~\cite{li2017knowledge} investigate the correctness of a fact by searching for evidences in other knowledge bases, web data, and searching logs. 
Similarly, \cite{lehmann2012defacto} suggests individual checking of a single facts in different datasets in order to detect inaccurate facts.
This is also useful for yielding larger-scale gold standards, but has two sources of errors: errors in the target knowledge graph, and errors in the linkage between the two.
\end{itemize}
